CAMIL: Context-Aware Multiple Instance Learning for Cancer Detection and Subtyping in Whole Slide Images

The visual examination of tissue biopsy sections is fundamental for cancer diagnosis, with pathologists analyzing sections at multiple magnifications to discern tumor cells and their subtypes. However, existing attention-based multiple instance learning (MIL) models used for analyzing Whole Slide Images (WSIs) in cancer diagnostics often overlook the contextual information of tumor and neighboring tiles, leading to misclassifications. To address this, we propose the Context-Aware Multiple Instance Learning (CAMIL) architecture. CAMIL incorporates neighbor-constrained attention to consider dependencies among tiles within a WSI and integrates contextual constraints as prior knowledge into the MIL model. We evaluated CAMIL on subtyping non-small cell lung cancer (TCGA-NSCLC) and detecting lymph node (CAMELYON16 and CAMELYON17) metastasis, achieving test AUCs of 97.5\%, 95.9\%, and 88.1\%, respectively, outperforming other state-of-the-art methods. Additionally, CAMIL enhances model interpretability by identifying regions of high diagnostic value.

==> removed_tex.tex <==
\begin{table}[htb!]
    \centering
    \caption{Classification results on CAMELYON16 and TCGA-NSCL}
    \label{tab:results}
    \begin{tabular}{lcccc}
    \hline
    & \multicolumn{2}{c}{CAMELYON16} & \multicolumn{2}{c}{TCGA-NSCLC} \\
    \cline{2-3} \cline{4-5}
    METHOD & ACC($\uparrow$)  & AUC($\uparrow$) & ACC($\uparrow$) & AUC($\uparrow$)\\
    \hline
        Mean-pool & 0.713 \tiny$0.027$ & 0.695\tiny${0.005}$ & 0.822\tiny${ 0.039}$  & 0.934\tiny${0.004}$ \\
        Max-pool  &0.841\tiny${0.026}$ & 0.921\tiny${ 0.001}$  & 0.888\tiny${ 0.002}$ & 0.956\tiny${0.002}$ \\
        CLAM-SB & 0.877\tiny${ 0.029}$  & 0.933\tiny${0.002}$ &0.903\tiny${0.011}$ & 0.972\tiny${0.004}$\\
        CLAM-MB & 0.894\tiny${0.010}$  & 0.938\tiny${0.005}$ &0.904\tiny${ 0.010}$  & 0.973\tiny${ 0.004}$ \\
        TransMIL & 0.905\tiny${0.005}$ & 0.950\tiny${0.005}$ &0.905\tiny${0.011}$& 0.974\tiny${0.003}$ \\
        DTFD-MIL & 0.889\tiny${0.007}$ &  0.941\tiny${0.005}$ &0.899\tiny${0.010}$  & 0.964\tiny${0.003}$ \\  
        GTP & 0.883\tiny${0.026}$  &  0.921\tiny${0.026}$ &\bfseries{0.916}\tiny${0.015}$  &  0.973\tiny${0.006}$\\
        \hline & \\[-1.5ex]
        \bfseries {CAMIL-L} & 0.910\tiny${0.010}$  &  0.953\tiny${0.002}$ &0.914\tiny${0.011}$ &  0.975\tiny${0.004}$\\
        \bfseries {CAMIL-G} & 0.891\tiny${0.001}$  &  0.950\tiny${0.009}$ &0.907\tiny${0.012}$  &  0.973\tiny${0.004}$\\
        \bfseries {CAMIL} & \bfseries{0.917\tiny${ 0.006}$} & \bfseries{0.959}\tiny${0.001}$ &\bfseries{0.916}\tiny${0.007}$ & \bfseries{0.975}\tiny${ 0.003}$ \\
    \hline
    \end{tabular}
\end{table}

=========================================================

CAMIL outperforms all existing MIL models on the CAMELYON16 cancer dataset across all evaluation metrics.  Importantly, in the CAMELYON16 dataset, tumor cells may account for as little as 5\% of any WSI. The low frequency of tumor cells in tissue samples is particularly common \citep{cheng_computational_2021} to metastatic sites, where tumor cells are interspersed within large regions of normal cells. Thus, CAMIL - which re-adjusts the attention coefficients by inspecting a tile's neighborhood - was more effective at identifying clinically relevant, sparse, cancerous regions amidst a sea of normal cells than other models. Specifically, CAMIL outperforms the other baseline models on the CAMELYON16 dataset by significant margins, achieving at least 0.9\% better in the AUC and 1.2\% in ACC than the existing models.

In the TCGA-NSCLC, CAMIL achieved the highest performance on par with the GTP model (in terms of ACC). Notably, the GTP model, which incorporates a MinCUT pooling layer \citep{bianchi2019mincut}, performs effectively in this dataset but not in the CAMELYON16 dataset. The purpose of the MinCUT pooling layer is to reduce the memory and time complexity of the self-attention mechanism in the transformer layer. Reducing the number of nodes in the graph from thousands to hundreds makes the self-attention computation more manageable. However, the CAMELYON16 dataset is large and complex, and this pooling operation may result in information loss, particularly in retaining fine-grained details. On the contrary, the relatively smaller dataset size of TCGA-NSCLC allows the GTP model to retain sufficient information and remain competitive even after the MinCUT pooling operation.

CAMIL outperforms all the baseline models in both ACC and AUC metrics. Notably, the GTP model didn't perform well on this dataset, possibly due to its size, as was the case with CAMELYON16. We suspect that this drop in performance could be attributed to the MinCut pooling [3] operation, which could result in substantial information loss. Interestingly, DTFD-MIL performed very well, leveraging the power of pseudo-bags, which could be very beneficial when dealing with WSIs containing many tiles. As expected, Tranmil's performance is similar to CAMIL-G, since both models use the same Nystromformer architecture. We presume that the superiority of CAMIL-G performance over TransMIL in accuracy might arise from the distinct aggregation strategies they employ, with CAMIL-G model utilizing attention pooling before classifier input. Finally, the amalgamation of both elements in the CAMIL model yields the best performance overall.

=======================================

CAMIL outperforms all other MIL models on the CAMELYON16, TCGA-NSCLC, and CAMELYON17 datasets regarding ACC and AUC, except for DTFD-MIL on CAMELYON17 in AUC with a 0.003 difference. In the CAMELYON16 dataset, tumor cells may account for as little as 5\% of any WSI. The low frequency of tumor cells in tissue samples is particularly common in metastatic sites \citep{cheng_computational_2021}, where tumor cells are interspersed within large regions of normal cells. Thus, CAMIL - which re-adjusts the attention coefficients by inspecting a tile's neighborhood - was more effective at identifying clinically relevant, sparse, cancerous regions amidst a sea of normal cells than other models.

GTP, which incorporates a MinCUT pooling layer \citep{bianchi2019mincut}, performs effectively on TGCA-NSCLC but not on CAMELYON16 or CAMELYON17. The purpose of the MinCUT pooling layer is to reduce the memory and time complexity of the self-attention mechanism in the transformer layer. Reducing the number of nodes in the graph from thousands to hundreds makes the self-attention computation more manageable. However, the CAMELYON16 and CAMELYON17 datasets are large and complex, and this pooling operation may result in information loss, particularly in retaining fine-grained details. On the contrary, the relatively smaller dataset size of TCGA-NSCLC allows the GTP model to retain sufficient information and remain competitive even after the MinCUT pooling operation.

DTFD-MIL performed well on CAMELYON16 and CAMELYON17 regarding AUC, leveraging the power of pseudo-bags, which could be very beneficial when dealing with WSIs containing many tiles. As expected, TransMIL's performance is similar to CAMIL-G across datasets since both models use the same Nystromformer architecture. We presume that the superiority of CAMIL-G performance over TransMIL in accuracy might arise from the distinct aggregation strategies they employ, with CAMIL-G model utilizing attention pooling before classifier input. Finally, the amalgamation of both elements in the CAMIL model yields the best performance overall.


=================================================

We also qualitatively compared our model with the graph-based method, GTP, and the transformer-based histopathology framework, TransMIL. Similarly to our model, both methods retain spatial information to enhance predictions at the whole slide image (WSI) level. GTP uses GraphCAM to propagate the transformer attention maps and class relevance scores through the network. It then reconstructs the class activation map for the entire WSI using its graph representation. TransMIL utilizes a transformer to generate an attention matrix whose class token corresponds to the attention coefficients of every tile within a WSI. This method also leverages spatial information in its analysis of histopathology data.




========================================
To encode the feature embeddings $\boldsymbol{H} = \{\boldsymbol{h}_1, \ldots, \boldsymbol{h}_i, \ldots, \boldsymbol{h}_N\}, \boldsymbol{h}_i \in \mathbb{R}^{n \times d} $, we use a transformer layer, denoted as $T(\boldsymbol{h})$ in Figure \ref{fig:my_model}. CAMIL leverages the transformer layer to capture the relationships and dependencies between the tiles, enhance the understanding of the global context, and facilitate a more comprehensive feature aggregation. To circumvent the memory overload associated with the long-range dependencies of large WSIs, we adopt the Nystromformer architecture \citep{DBLP:conf/aaai/XiongZCTFLS21} to model feature interactions that otherwise would be intractable. The approximate self-attention mechanism can be defined as follows:

\begin{equation*}
\text{g} = \text{softmax}\Bigg(\frac{\boldsymbol{Q}_1 \boldsymbol{\Tilde{K}}_1^{T}} {\sqrt{\text{d}_\text{k}}}\Bigg)
\Bigg( \boldsymbol{A} \Bigg)^+
\text{softmax}\Bigg(\frac{\boldsymbol{\Tilde{Q}}_1 \boldsymbol{K}_1^{T}} {\sqrt{\text{d}_\text{k}}}\Bigg)\boldsymbol{V},
\end{equation*}
where $\boldsymbol{\Tilde{Q}}_1$ and $\boldsymbol{\Tilde{K}}_1$ are the $m$ selected landmarks from the original $n$-dimensional sequence of $\boldsymbol{Q}_1$ and $\boldsymbol{K}_1$, $ \boldsymbol{A}^+=\text{softmax}\Bigg(\frac{\boldsymbol{\Tilde{Q}}_1 \boldsymbol{\Tilde{K}}_1^{T}} {\sqrt{\text{d}_\text{k}}}\Bigg)^+ $ is the approximate inverse of $\boldsymbol{A}$, and softmax is applied along the rows of the matrix.




===============================================
related work


Typically, to serve as input for a deep neural network (DNN), a WSI is divided into non-overlapping fixed-size tiles, which are assigned a weak label based on the slide-level diagnosis. Under the MIL formulation, the prediction of a WSI label (i.e., cancerous or not) can come either directly from the tile predictions \citep{Campanella2019ClinicalgradeCP,10.1093/bioinformatics/btaa847,DBLP:conf/cvpr/HouSKGDS16,DBLP:conf/iccv/XuSSKYLWMX19}, or from a higher-level bag representation resulting from the aggregation of the tile features \citep{DBLP:conf/icml/IlseTW18,DBLP:journals/corr/abs-2004-09666,DBLP:conf/midl/SharmaSEMSB21,DBLP:journals/pr/WangYTBL18}. The former approach is referred to as instance based. The latter, known as the bag embedding-based approach, has empirically demonstrated superior performance \citep{DBLP:conf/midl/SharmaSEMSB21,DBLP:journals/pr/WangYTBL18}. Most recent bag embedding-based approaches employ attention mechanisms \citep{DBLP:conf/nips/VaswaniSPUJGKP17}, which assign an attention score to every tile reflecting its relative contribution to the collective WSI-level representation. Attention scores enable the automatic localization of sub-regions of high diagnostic value in addition to informing the WSI-level label \citep{
DBLP:conf/cvpr/ZhangMAGSVS21,
DBLP:conf/miccai/BenTaiebH18,
DBLP:journals/corr/abs-2004-09666}. 

Attention-based MIL models vary in how they explore tissue structure in WSIs. Many are permutation invariant, assuming the tiles are independent and identically distributed. Building upon this assumption,  \citet{DBLP:conf/icml/IlseTW18} proposed a learnable attention-based MIL pooling operator that computes the bag embedding as the average of all tile features in the WSI weighted by their respective attention score. This operator has been widely adopted and modified with the addition of a clustering layer \citep{DBLP:journals/corr/abs-2004-09666,DBLP:journals/cbm/LiLSYWSA21,DBLP:journals/mia/YaoZJHH20} to further encourage the learning of semantically-rich, separable and class-specific features. Another variation of the same model uses `pseudo bags' \citep{DBLP:conf/cvpr/ZhangMZQYCZ22}. The original bag (WSI) can be split into several smaller bags to alleviate the issue of the limited number of training data.

However, permutation invariant operators cannot inherently capture the structural dependencies among different tiles at the input. The lack of bio-topological information has partially been remedied by the introduction of feature similarity scores instead of positional encodings to model the mutual tile dependencies within a WSI \citep{DBLP:conf/midl/XieMVCYCF20,DBLP:journals/pami/TellezLLC21,DBLP:conf/cvpr/AdnanKT20}. For instance, DSMIL \citep{DBLP:journals/corr/abs-2011-08939} utilizes a non-local operator to compute an attention score for each tile by measuring the similarity of its feature representation against that of a critical tile. Recently, to consider the correlations between the different tiles of a WSI, transformer-based architectures have been introduced, which usually make use of a learnable position-dependent signal to incorporate the spatial information of the image \citep{DBLP:conf/cvpr/ZhaoYFLZZSYMFY20,DBLP:journals/corr/abs-1906-04881}. For instance, TransMIL \citep{DBLP:conf/nips/ShaoBCWZJZ21} is a transformer-like architecture trained end-to-end to optimize for the classification task and produce attention scores while simultaneously learning the positional embeddings. %add a citation here where transformers miss the underlying biological patterns 

In CAMIL, we provide explicit guidance regarding the context of every tile as we argue that it can provide a valuable, rich source of information. Unlike most existing MIL approaches where the relationships developed between neighboring tiles are omitted, in our approach, we propose a neural network architecture that explicitlyleverages the dependencies between neighboring tiles of a WSI by enforcing bio-topological constraints to enhance performance effectively. 


We sought to determine if CAMIL can effectively capture informative context relationships and, if so, determine whether those relationships can improve MIL performance in terms of classification and localization. To this end, we evaluated CAMIL on three histopathology datasets.

\subsection{Datasets}\label{sec:results}

We conducted a series of experiments in three publicly available and widely-used histopathology datasets: CAMELYON16 \citep{ehteshami_bejnordi_diagnostic_2017}, CAMELYON17 \cite{8447230}, and TCGA-NSCLC. Additional information about the datasets, including details about the training and test sets and our baseline models, can be found in the appendix.
